Meta-Learning Stationary Stochastic Process Prediction with Convolutional Neural Processes

Stationary stochastic processes (SPs) are a key component of many probabilistic models, such as those for off-the-grid spatio-temporal data. They enable the statistical symmetry of underlying physical phenomena to be leveraged, thereby aiding generalization. Prediction in such models can be viewed as a translation equivariant map from observed data sets to predictive SPs, emphasizing the intimate relationship between stationarity and equivariance. Building on this, we propose the Convolutional Neural Process (ConvNP), which endows Neural Processes (NPs) with translation equivariance and extends convolutional conditional NPs to allow for dependencies in the predictive distribution. The latter enables ConvNPs to be deployed in settings which require coherent samples, such as Thompson sampling or conditional image completion. Moreover, we propose a new maximum-likelihood objective to replace the standard ELBO objective in NPs, which conceptually simplifies the framework and empirically improves performance. We demonstrate the strong performance and generalization capabilities of ConvNPs on 1D regression, image completion, and various tasks with real-world spatio-temporal data.

==> arxiv_camera_ready_full copy/diagrams/forward_pass.tex <==
% Source: https://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,color=white,fill=black,draw,inner sep=1pt] (char) {#1};}}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{plots/gp1d/forward_pass.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [anchor=south] () at (-11.8cm, 2cm) {\scriptsize \circled{\textbf{1}}\hspace{5 pt}Context set $D_c$};
        \node [anchor=south] () at (-7cm, 2cm) {\scriptsize \circled{\textbf{2}}\hspace{5 pt}Encoder: $z \sim \mathrm{ConvCNP}(D_c)$};
        \node [anchor=south] () at (-2cm, 2cm) {\scriptsize \circled{\textbf{3}}\hspace{5 pt}Decoder: $f = d(z)$};
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-9.6cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{E}_\vphi$
        } (-9.25cm, 0.9cm);
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-4.7cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{D}_\vtheta$
        } (-4.35cm, 0.9cm);
    \end{tikzpicture}%
    \caption{
        Encoder-decoder architecture. The ConvCNP encoder takes the context set as input (left panel) and outputs a single sample of $z$ (center panel). The decoder takes this as input and outputs a predictive sample (right panel blue; two other samples shown in grey).
    }
    \label{fig:forward_pass}
    %\vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/diagrams/forwardpass_full.tex <==
% Source: https://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,color=white,fill=black,draw,inner sep=1pt] (char) {#1};}}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{plots/gp1d/forward_pass.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [anchor=south] () at (-11.8cm, 2cm) {\scriptsize \circled{\textbf{1}}\hspace{5 pt}Context set $D_c$};
        \node [anchor=south] () at (-7cm, 2cm) {\scriptsize \circled{\textbf{2}}\hspace{5 pt}Encoder: $z \sim \mathrm{ConvCNP}(D_c)$};
        \node [anchor=south] () at (-2cm, 2cm) {\scriptsize \circled{\textbf{3}}\hspace{5 pt}Decoder: $f = d(z)$};
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-9.6cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{E}_\vphi$
        } (-9.25cm, 0.9cm);
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-4.7cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{D}_\vtheta$
        } (-4.35cm, 0.9cm);
    \end{tikzpicture}%
    \caption{
        ConvNP encoder-decoder architecture. The encoder is a ConvCNP which takes the context set as input (left panel) and outputs a single sample of $z$ (center panel). The decoder takes this as input and outputs a predictive sample (right panel blue; two other samples shown in grey).
    }
    \label{fig:forward_pass}
    %\vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> arxiv_camera_ready_full copy/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\rtau{{\textnormal{$\tau$}}}
\def\rtheta{{\textnormal{$\theta$}}}
\def\rbeta{{\textnormal{$\beta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\boldsymbol{\epsilon}}}
\def\rvtheta{{\boldsymbol{\theta}}}
\def\rvlambda{{\boldsymbol{\lambda}}}
\def\rvdelta{{\boldsymbol{\delta}}}
\def\rvbeta{{\boldsymbol{\beta}}}
\def\rvtau{{\boldsymbol{\tau}}}
\def\rvmu{{\boldsymbol{\mu}}}
\def\rvphi{{\boldsymbol{\phi}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}
\def\vtheta{{\bm{\theta}}}
\def\vlambda{{\bm{\lambda}}}
\def\vbeta{{\bm{\beta}}}
\def\veta{{\bm{\eta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vdelta{{\bm{\delta}}}
\def\vphi{{\bm{\phi}}}
\def\vpsi{{\bm{\psi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\mOmega{{\bm{\Omega}}}
\def\mDelta{{\bm{\Delta}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arxiv_camera_ready_full copy/plots/bayes_opt_plot.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=1.\textwidth]{plots/environmental/bayesopt/bayes_opt_plot.pdf}%
    \vspace*{-4pt}%
    \caption{Average regret plotted against number of points queried, averaged over 5000 tasks.}
    \label{fig:bayesopt}
    %\vspace*{-1em}
\end{figure}

==> arxiv_camera_ready_full copy/plots/europe_regions.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\textwidth]{plots/environmental/europe.png}
    \caption{Training (blue) and test (red) regions in Europe, along with orography data from ERA5Land.}
    \label{fig:eu_data_regions}
\end{figure}

==> arxiv_camera_ready_full copy/plots/gp_plots_1d.tex <==
\begin{figure}
    \centering
    \makebox[0.49\linewidth][c]{\textsc{ConvNP}}
    \hfill \makebox[0.49\linewidth][c]{\textsc{ANP}} \\[2pt]
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=south] () at (0, 0) {\tiny\textsc{Mat\'ern--$\frac52$}};
    \end{tikzpicture}%
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_loglik_matern52_within.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_loglik_matern52_within.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{ML}}$};
    \end{tikzpicture}\\
    %
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_elbo_matern52_within.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_elbo_matern52_within.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{NP}}$};
    \end{tikzpicture}\\
    %
    %
    %
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=south] () at (0, 0) {\tiny\textsc{Mat\'ern--$\frac52$}};
    \end{tikzpicture}%
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_loglik_matern52_outside.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_loglik_matern52_outside.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{ML}}$};
    \end{tikzpicture}\\
    %
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_elbo_matern52_outside.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_elbo_matern52_outside.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{NP}}$};
    \end{tikzpicture}\\
    %
    %
    %
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=south] () at (0, 0) {\tiny\textsc{Weakly Periodic}};
    \end{tikzpicture}%
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_loglik_weakly-periodic_within.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_loglik_weakly-periodic_within.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{ML}}$};
    \end{tikzpicture}\\
    %
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_elbo_weakly-periodic_within.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_elbo_weakly-periodic_within.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{NP}}$};
    \end{tikzpicture}\\
    %
    %
    %
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=south] () at (0, 0) {\tiny\textsc{Sawtooth}};
    \end{tikzpicture}%
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_loglik_sawtooth_outside.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_loglik_sawtooth_outside.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{ML}}$};
    \end{tikzpicture}\\
    %
    \includegraphics[width=0.49\linewidth]{plots/gp1d/convnp-het_elbo_sawtooth_outside.pdf}
    \hfill \includegraphics[width=0.49\linewidth]{plots/gp1d/anp-het_elbo_sawtooth_outside.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [rotate=90, anchor=north] () at (0, 15pt) {\tiny $\gL_{\mathrm{NP}}$};
    \end{tikzpicture}
    \caption{
        Predictions of ConvNPs and ANPs trained with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$, showing interpolation and extrapolation within (grey background) and outside (white background) the training range. Solid blue lines are samples, dashed blue lines are means, and the shaded blue area is $\mu \pm 2\sigma$. Purple dash--dot lines are the ground-truth GP mean and $\mu\pm2\sigma$. ConvNP handles points outside the training range naturally, whereas this leads to catastrophic failure for the ANP. Note ANP with $\gL_{\mathrm{NP}}$ tends to collapse to deterministic samples, with all uncertainty explained with the heteroskedastic noise. In contrast, models trained with $\gL_{\mathrm{ML}}$ show diverse samples that account for much of the uncertainty. 
    }
    \label{fig:1D_predictions}
    \vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/plots/image_completion/data/zsmm_data.tex <==
\begin{figure}[htb]
\centering
\begin{subfigure}{0.40\textwidth}
  \includegraphics[width=\linewidth]{plots/image_completion/data/zsmm_train.png}
  \subcaption{Train ($32  \times 32)$}
  \label{fig:zsmm_train}
\end{subfigure}
\begin{subfigure}{0.40\textwidth}
  \includegraphics[width=\linewidth]{plots/image_completion/data/zsmm_test.png}
  \subcaption{Test ($56 \times 56)$}
  \label{fig:zsmm_test}
\end{subfigure}

\caption{Samples from our generated Zero Shot Multi MNIST (ZSMM) data set.}
\label{fig:zsmm}
\end{figure}

==> arxiv_camera_ready_full copy/plots/image_completion/image_figures_hetero.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}[b]{0.43\textwidth}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_convnp_hetero.png}
        \subcaption{ConvNP}
        \label{fig:images_zsmm_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_anp_hetero.png}
        \subcaption{ANP}
        \label{fig:images_zsmm_anp}
    \end{subfigure}
    %
\end{subfigure}
%
\begin{subfigure}[b]{0.56\textwidth}
%
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp_hetero.png}
        \subcaption{ConvNP}
        \label{fig:images_marginal_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_anp_hetero.png}
        \subcaption{ANP}
        \label{fig:images_marginal_anp}
    \end{subfigure}
%
\end{subfigure}
%
\caption{Left two plots: predictive samples on zero-shot multi MNIST. Right two plots: samples and marginal predictives on standard MNIST. We plot the density of the five marginals that maximize Sarle's bimodality coefficient \cite{ellison1987effect}. We use $\gL_{\mathrm{ML}}$ for training.
Blue pixels are not in the context set.}
\label{fig:images_zsmm}
%\vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/plots/image_completion/image_figures_homo.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}[b]{0.43\textwidth}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_convnp_homo.png}
        \subcaption{ConvNP}
        \label{fig:images_zsmm_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_anp_homo.png}
        \subcaption{ANP}
        \label{fig:images_zsmm_anp}
    \end{subfigure}
    %
\end{subfigure}
%
\begin{subfigure}[b]{0.56\textwidth}
%
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp.png}
        \subcaption{ConvNP}
        \label{fig:images_marginal_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_anp.png}
        \subcaption{ANP}
        \label{fig:images_marginal_anp}
    \end{subfigure}
%
\end{subfigure}
%
\caption{Left two plots: predictive samples on zero-shot multi MNIST. Right two plots: samples and marginal predictives on standard MNIST. We plot the density of the five marginals that maximize Sarle's bimodality coefficient \cite{ellison1987effect}. We use $\gL_{\mathrm{ML}}$ for training.
Blue pixels are not in the context set.}
\label{fig:images_zsmm}
%\vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/plots/image_completion/marginal/marginal_pred.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}{0.49\columnwidth}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp.png}
%\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp.png}
\end{subfigure}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_convnp.png}
\end{subfigure} 
\subcaption{ConvNP}
\label{fig:images_marginal_convnp}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_anp.png}
%\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_anp.png}
\end{subfigure}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_anp.png}
\end{subfigure}
\subcaption{ANP}
\label{fig:images_marginal_anp}
\end{subfigure}
\caption{Samples and associated marginal predictives from (a) ConvNP and (b) ANP. 
We selected marginal predictive that were multi-modal by considering the seven ones that maximize Sarle's bimodality coefficient \cite{ellison1987effect}. Blue pixels correspond to the ones that are not in the context set. 
}
\label{fig:images_marginal_pred}
\end{figure}

==> arxiv_camera_ready_full copy/plots/image_completion/zsmm/zsmm.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}{0.27\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_convnp.png}
\subcaption{ConvNP}
\label{fig:images_zsmm_convnp}
\end{subfigure}
\begin{subfigure}{0.27\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_anp.png}
\subcaption{ANP}
\label{fig:images_zsmm_anp}
\end{subfigure}
\caption{Samples from the ANP and ConvNP in a zero-shot spatial generalization task, where the models are trained on single digits and tested on multiple digits. 
}
\label{fig:images_zsmm}
\end{figure}

==> arxiv_camera_ready_full copy/plots/kde_plots.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\textwidth]{plots/environmental/KDE/kde_pixel0.png}
        \subcaption{}
        \label{fig:pred_density_sparse}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\textwidth]{plots/environmental/KDE/kde_pixel450.png}
        \subcaption{}
        \label{fig:pred_density_asymm}
    \end{subfigure}
    \caption{Predictive density at two target points, where the ConvNP significantly outperforms the GP. The orange and blue circles show the likelihood of the ground truth target value under the GP and ConvNP. Note that as the precipitation values are normalized to zero mean and unit standard deviation, $y_t = -0.53$ corresponds to no rain. In \cref{fig:pred_density_sparse}, we see the ConvNP sometimes produces predictions heavily centered on this value, showing it has learned the sparsity of precipitation values. In \cref{fig:pred_density_asymm} we see the ConvNP predictive distribution is sometimes asymmetric with a heavier positive tail, reflecting the non-negativity of precipitation.}
    \label{fig:pred_density}
\end{figure}

==> arxiv_camera_ready_full copy/plots/percipitation_samples.tex <==
\begin{figure}[th!]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/ground_truth.png}
  \label{fig:ground_truth}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/np_sample0.png}
  \label{fig:np_sample1}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/np_sample1.png}
  \label{fig:np_sample2}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/np_sample2.png}
  \label{fig:np_sample3}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/context_set.png}
  \label{fig:context_Set}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/gp_sample0.png}
  \label{fig:gp_sample1}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/gp_sample1.png}
  \label{fig:gp_sample2}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/main40x40/gp_sample2.png}
  \label{fig:gp_sample3}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Predictive samples overlaid on central Europe. Darker colours show higher precipitation. In (e), coloured pixels represent context points. GP samples often take negative values (lighter than ground truth data, see \cref{app:environmental_gp_baselines} for a discussion), whereas the NP has learned to produce non-negative samples which capture the \emph{sparsity} of precipitation. The model is trained on subregions roughly the size of the lengthscale of the precipitation process. More samples in \cref{app:environmental_figures}.}
\label{fig:precipitation_example_task}
%\vspace*{-1.5em}
\end{figure}

==> arxiv_camera_ready_full copy/plots/perf_v_samples/perf_v_samples.tex <==
\begin{figure}[t]
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=.9\textwidth]{plots/perf_v_samples/samples_eval_matern52.pdf}
    \caption{Mat\'ern--$\frac52$}
    \label{fig:perf_v_samples_matern}
\end{subfigure}
%
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=.9\textwidth]{plots/perf_v_samples/samples_eval_weakly-periodic.pdf}
    \caption{Weakly periodic kernel}
    \label{fig:perf_v_samples_weakly-periodic}
\end{subfigure}
\caption{
    Log-likelihood bounds achieved by various combination of models and training objectives when evaluated with $\gL_{\textrm{ML}}$ and $\gL_{\textrm{IW}}$ for various numbers of samples $L$.
    Color indicates model.
    Solid lines correspond to models trained and evaluated with $\gL_{\textrm{ML}}$.
    Dashed lines correspond to models trained with $\gL_{\textrm{NP}}$ and evaluated with $\gL_{\textrm{IW}}$.
    Dotted lines correspond to models trained with $\gL_{\textrm{ML}}$ and evaluated with $\gL_{\textrm{ML}}$.
    % Color-coding indicates model / loss pairs, solid lines denote evaluation with $\gL_{\textrm{ML}}$, and dashed lines denote evaluation with $\gL_{\textrm{IW}}$. Performance of ConvNP when trained with $\gL_{\textrm{NP}}$ and evaluated with $\gL_{\textrm{ML}}$ is plotted separately for each kernel to allow for the different scales.
}
\label{fig:perf_v_samples}
\end{figure}

==> arxiv_camera_ready_full copy/plots/prec_samples/prec_samples_app_28x28.tex <==
\begin{figure}[t]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/ground_truth.png}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/np_sample0.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/np_sample1.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/np_sample2.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/context_set.png}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/gp_sample0.png}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/gp_sample1.png}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28/gp_sample2.png}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Samples from the predictive processes overlaid on central Europe, for  a model trained on random $28 \times 28$ subregions of the full $61 \times 201$ central Europe region. Note some blocky artefacts in the ConvNP samples due to training on small subregions. Here the GP has overfit to the orography data, with samples that resemble the orography rather than precipitation.}
\label{fig:precipitation_sample_28x28}
\end{figure}

==> arxiv_camera_ready_full copy/plots/prec_samples/prec_samples_app_28x28_2.tex <==
\begin{figure}[th!]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/ground_truth.png}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/np_sample0.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/np_sample1.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/np_sample2.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/context_set.png}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/gp_sample0.png}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/gp_sample1.png}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app28x28_2/gp_sample2.png}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Samples from the predictive processes overlaid on central Europe, for  a model trained on random $28 \times 28$ subregions of the full $61 \times 201$ central Europe region. Here the GP has learned a lengthscale that is too large.}
\label{fig:precipitation_sample_28x28_2}
\end{figure}

==> arxiv_camera_ready_full copy/plots/prec_samples/prec_samples_app_40x40.tex <==
\begin{figure}[t]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/ground_truth.png}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/np_sample0.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/np_sample1.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/np_sample2.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/context_set.png}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/gp_sample0.png}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/gp_sample1.png}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40/gp_sample2.png}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Samples from the predictive processes overlaid on central Europe, for a model trained on random $40 \times 40$ subregions of the full $61 \times 201$ central Europe region. Here the GP has overfit to the orography data, with samples that resemble the orography rather than precipitation.}
\label{fig:precipitation_sample_40x40}
\end{figure}

==> arxiv_camera_ready_full copy/plots/prec_samples/prec_samples_app_40x40_2.tex <==
\begin{figure}[t]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/ground_truth.png}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/np_sample0.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/np_sample1.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/np_sample2.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/context_set.png}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/gp_sample0.png}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/gp_sample1.png}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_2/gp_sample2.png}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Samples from the predictive processes overlaid on central Europe, for a model trained on random $40 \times 40$ subregions of the full $61 \times 201$ central Europe region. The GP has again overfit to the orography data.}
\label{fig:precipitation_sample_40x40_2}
\end{figure}

==> arxiv_camera_ready_full copy/plots/prec_samples/prec_samples_app_40x40_3.tex <==
\begin{figure}[t]
%%
     %%%  First row: Ground truth and NP samples  %%%
%%
\vspace*{-0.8em}
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/ground_truth.png}
  \vspace{-1.5em}
  \caption{Ground truth data}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/np_sample0.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 1}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/np_sample1.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 2}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/np_sample2.png}
  \vspace{-1.5em}
  \caption{ConvNP sample 3}
\end{subfigure}\\
%%
     %%%  Second row: Context set and GP samples  %%%
%%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/context_set.png}
  \vspace{-1.5em}
  \caption{Context set}
\end{subfigure}\hfil 
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/gp_sample0.png}
  \vspace{-1.5em}
  \caption{GP sample 1}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/gp_sample1.png}
  \vspace{-1.5em}
  \caption{GP sample 2}
\end{subfigure}\hfil
%
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{plots/environmental/samples/app40x40_3/gp_sample2.png}
  \vspace{-1.5em}
  \caption{GP sample 3}
\end{subfigure}
%
\caption{Samples from the predictive processes overlaid on central Europe, for a model trained on random $40 \times 40$ subregions of the full $61 \times 201$ central Europe region.}
\label{fig:precipitation_sample_40x40_3}
\end{figure}

==> arxiv_camera_ready_full copy/preamble.tex <==
%auto-ignore
\usepackage[T1]{fontenc}    % Use 8-bit T1 fonts

% Some common commands
\newcommand{\Versa}{\textsc{Versa}}
\renewcommand{\d}{\mathrm{d}}

% Bibliography management
%\usepackage[]{natbib}
%\renewcommand{\bibname}{References}
%\renewcommand{\bibsection}{\subsubsection*{\bibname}}

\usepackage{microtype}      % Microtypography
\usepackage[utf8]{inputenc} % Allow utf-8 input
\usepackage{hyperref}       % Hyperlinks
\usepackage{url}            % Simple URL typesetting
\usepackage{booktabs}       % Professional-quality tables
\usepackage{multirow}       % Helper package for organizing tables    
\usepackage{amsfonts}       % Blackboard math symbols
\usepackage{nicefrac}       % Compact symbols for 1/2, etc.
\usepackage{tabularx}       % Tables
\usepackage{makecell}       % More for tables
\usepackage{ragged2e}       % Justification
\usepackage{paralist}       % Compact lists
\usepackage{arydshln}       % Dashed lines in tables
\usepackage{xargs}          % Use more than one optional parameter in a new commands
\usepackage{color, colortbl}
% Add labeled todo-notes and comments
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
% \usepackage{algorithm}      % http://ctan.org/pkg/algorithm
% \usepackage{algpseudocode}  % http://ctan.org/pkg/algorithmicx
% \usepackage[linesnumbered]{algorithm2e}    % For writing algorithms
\usepackage{xparse}
\NewDocumentCommand{\scnum}{ >{\SplitArgument{1}{e}}m }
 {\scnumaux#1}
 \NewDocumentCommand{\scnumaux}{ m m }
 {#1\,\mathrm e\,{#2}}

\usepackage{import}         % Importing subdocuments
\usepackage{standalone}     % Compilable subdocuments and inclusion thereof
%\usepackage{titlesec}       % Tweak titles
\usepackage{enumitem}
  \newlist{inlinelist}{enumerate*}{1}
  \setlist*[inlinelist,1]{%
          label=(\roman*),
      }

\usepackage{amsmath}
\usepackage{cases}          % Cases in math
\usepackage{amsthm}         % Theorems
\usepackage{thmtools}       % Tools for theorems
\usepackage{mathtools}      % More math commands
%\usepackage{subcaption}     % Subcaptions

\usepackage{pgf}
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.13}

\usepgfplotslibrary{groupplots}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{angles,quotes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{external}
\usetikzlibrary{fit}
\usetikzlibrary{bayesnet}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{spy, shadows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shadings}
\usetikzlibrary{fadings}
%\usetikzlibrary{tikzmark}
\usetikzlibrary{matrix}     % SI units
\usepackage[
    capitalize,
    nameinlink]{cleveref}   % Automatic referencing

% Draw an open plus.
\DeclareRobustCommand{\openplus}{%
    \begin{tikzpicture}[baseline=-.8ex, line width=.5, scale=0.075]
        \draw (0,0) -- (0,1) -- (1,1) -- (1,0) -- (2,0) -- (2,-1) -- (1,-1) -- (1,-2) -- (0,-2) -- (0,-1) -- (-1,-1) -- (-1,0) -- cycle;
    \end{tikzpicture}%
}

% Fix interference of parfill option of parskip package with amsmath environments.
\begingroup
    \makeatletter
    \@for\theoremstyle:=theorem,corollary,lemma,model,definition,remark,plain\do{%
        \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
            \setlength\thm@preskip\parskip
            \setlength\thm@postskip\parskip%{0pt}
            \addtolength\thm@preskip\parskip
            }%
        }
    \makeatother
\endgroup

% Restatable theorems 
\usepackage{thmtools,thm-restate}
\newtheorem{lem}{Lem}
\newtheorem{thm}{Thm}
\newtheorem{prop}{Prop}

% Environments
\theoremstyle{definition}
\newtheorem{theorem}{Thm}
\newtheorem*{theorem*}{Thm}
\newtheorem{lemma}{Lem}
\newtheorem*{lemma*}{Lem}
\newtheorem{remark}{Rem}
\newtheorem*{remark*}{Rem}
\newtheorem{definition}{Def}
\newtheorem*{definition*}{Def}
\newtheorem{proposition}{Prop}
\newtheorem*{proposition*}{Prop}
\newtheorem{property}{Prop}
\newtheorem*{property*}{Prop}

% Cleverref environments
\crefname{thm}{Thm}{Thms}
\Crefname{thm}{Thm}{Thms}
\crefname{lem}{Lem}{Lems}
\Crefname{lem}{Lem}{Lems}
\crefname{proposition}{Prop}{Props}
\Crefname{proposition}{Prop}{Props}
\crefname{definition}{Def}{Defs}
\Crefname{definition}{Def}{Defs}
\crefname{property}{Prop}{Props}
\Crefname{property}{Prop}{Props}
\crefname{equation}{Eq}{Eqs}
\Crefname{equation}{Eq}{Eqs}
\crefname{section}{Sec}{Secs}
\Crefname{section}{Sec}{Secs}
\crefname{figure}{Fig}{Figs}
\Crefname{figure}{Fig}{Figs}
\crefname{table}{Tab}{Tabs}
\Crefname{table}{Tab}{Tabs}
\crefname{appendix}{App}{Apps}
\Crefname{appendix}{App}{Apps}

% Custom stuff
\newcommand{\ts}{\textsuperscript}

% Tabularx fields
\newcolumntype{L}{>{\RaggedRight\arraybackslash}X}

% Linear algebra
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}} % Vector
\newcommand{\mat}[1]{\vec{#1}}                   % Matrix
\renewcommand{\vec}[1]{#1}


% Commonly used sets
% \newcommand{\Z}{\mathbb{Z}}   % Integers
% \newcommand{\R}{\mathbb{R}}   % Real numbers
% \newcommand{\C}{\mathbb{C}}   % Complex numbers
% \newcommand{\N}{\mathbb{N}}   % Natural numbers

% Symbols
\newcommand{\es}{\varnothing}  % Empty set
\newcommand{\e}{\varepsilon}   % Epsilon
\newcommand{\sub}{\subseteq}   % Subset
\renewcommand{\d}{\partial}    % Partial
\renewcommand{\th}{\theta}     % Theta
\renewcommand{\O}{\mathcal{O}} % Landau's symbol


% Operators
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\max}{\operatorname{max}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\tr}{\operatorname{tr}}
%\newcommand{\sign}{\operatorname{sign}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\card}{\#}
\newcommand{\comp}{\circ}
\newcommand{\had}{\circ}
\newcommand{\chol}{\operatorname{chol}}
%\newcommand{\KL}{\operatorname{D}_{\text{KL}}}
\newcommand{\Top}{\operatorname{T}}

% Special math commands
\newcommand{\sd}[1]{\, \mathrm{d} #1}     % Straight 'd'
\newcommand{\sce}{\text{\sc{e}}}          % Scientific notation
\newcommand{\cond}{\, | \,}               % Conditioning
\newcommand{\set}[1]{\{#1\}}              % Set
\newcommand{\vardot}{\,\cdot\,}           % Dot for a variable
\newcommand{\T}{\text{\textsf{T}}}        % Transpose
\newcommand{\iidsim}{\overset{\raisebox{-2pt}{\smash{\text{\tiny i.i.d.}}}}{\sim}}  % Compact \sim with iid above it
\newcommand{\rlh}{\rightleftharpoons}     % Two-sided harpoons

% TikZ configuration
%\usetikzlibrary{arrows.meta, fit}
%\tikzset{
%    x = 4.5em,
%    y = 4em,
%    latent/.style = {
%        draw,
%        circle,
%        minimum size = 2.25em,
%        inner sep = 0pt
%    },
%    arrow/.style = {
%        -{Triangle[angle=45:.5em]}
%    },
%    plate/.style = {
%        draw,
%        shape = rectangle,
%        inner sep = 5pt,
%        rounded corners = 2pt
%    }
%}

% Colours:
\definecolor{tabgreen}{HTML}{59a14f}

% Define some naming 
\newcommand{\convcp}{\textsc{ConvCNP}}
\newcommand{\anp}{\textsc{AttnCNP}}


%\titlespacing{\section}{0pt}{.5\parskip}{.25\parskip}

% Add commenting for each collaborator
\newcommandx{\wpbnote}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{WPB: #2}}
\newcommandx{\jrrnote}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{JRR: #2}}
\newcommandx{\aykfnote}[2][1=]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple,#1]{AYKF: #2}}
\newcommandx{\jgnote}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{JG: #2}}
\newcommandx{\retnote}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{RET: #2}}
\newcommandx{\ydnote}[2][1=]{\todo[linecolor=orange,backgroundcolor=orange!25,bordercolor=orange,#1]{YD: #2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
\setlength{\marginparwidth}{3.4cm}

% Add commenting for each collaborator
% \newcommandx{\wpbnote}[2][1=]{}
% \newcommandx{\jrrnote}[2][1=]{}
% \newcommandx{\aykfnote}[2][1=]{}
% \newcommandx{\jgnote}[2][1=]{}
% \newcommandx{\retnote}[2][1=]{}
% \newcommandx{\ydnote}[2][1=]{}
% \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
% \setlength{\marginparwidth}{3.4cm}

==> arxiv_camera_ready_full copy/tables/bakeoff1d_amortised.tex <==
\begin{table}
\footnotesize
\caption{
    Log-likelihood for ConvCNP, ConvNP, ANP, and NP.
    Each of the stochastic models was trained on each data set with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$, separately.
    % The noise model for these experiments was \textit{amortized}.
}
\label{table:1d_bakeoff_amortized}
\begin{center}
\begin{tabular}{l@{\hspace{4pt}}l@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}

\toprule 
 & & \multicolumn{1}{c}{EQ} & \multicolumn{1}{c}{Mat\'ern--$\frac52$} & \multicolumn{1}{c}{Noisy Mixt.} & \multicolumn{1}{c}{Weakly Per.} & \multicolumn{1}{c}{Sawtooth}\\
\midrule\multicolumn{7}{l}{\textsc{Interpolation inside training range}} \\[0.5em] 
GP (full) & &
    $5.80 { \scriptstyle \,\pm\, 0.02 }$ &
    $1.22 { \scriptstyle \,\pm\, 6.3\text{\textsc{e}}{\,\text{--}3} }$ &
    $1.00 { \scriptstyle \,\pm\, 4.1\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}0.06 { \scriptstyle \,\pm\, 4.6\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
GP (diag) & &
    $\text{--}0.59 { \scriptstyle \,\pm\, 0.01 }$ &
    $\text{--}0.84 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}0.89 { \scriptstyle \,\pm\, 0.01 }$ &
    $\text{--}1.17 { \scriptstyle \,\pm\, 5.2\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
ConvCNP & & $\text{--}0.70 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.88 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.92 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}1.19 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $1.15 { \scriptstyle \,\pm\, 0.04 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{ML}}$ & $\text{--}0.30 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.58 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.55 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.02 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $2.30 { \scriptstyle \,\pm\, 0.01 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}0.52 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.73 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.69 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.14 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $0.09 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}0.84 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.96 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.93 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.23 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.02 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $\text{--}0.50 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.77 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.48 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}1.03 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ & $2.47 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}0.82 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.96 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.04 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.37 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $0.20 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}0.58 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.00 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.72 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.22 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.16 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\
\midrule\multicolumn{7}{l}{\textsc{Interpolation beyond training range}} \\[0.5em] 
GP (full) & &
    $5.80 { \scriptstyle \,\pm\, 0.02 }$ &
    $1.22 { \scriptstyle \,\pm\, 6.3\text{\textsc{e}}{\,\text{--}3} }$ &
    $1.00 { \scriptstyle \,\pm\, 4.1\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}0.06 { \scriptstyle \,\pm\, 4.6\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
GP (diag) & &
    $\text{--}0.59 { \scriptstyle \,\pm\, 0.01 }$ &
    $\text{--}0.84 { \scriptstyle \,\pm\, 9.0\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}0.89 { \scriptstyle \,\pm\, 0.01 }$ &
    $\text{--}1.17 { \scriptstyle \,\pm\, 5.2\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
ConvCNP & & $\text{--}0.69 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.87 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.94 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}1.19 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $1.11 { \scriptstyle \,\pm\, 0.04 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{ML}}$ & $\text{--}0.30 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.58 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.56 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.03 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $2.29 { \scriptstyle \,\pm\, 0.02 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}1.35 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.39 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.65 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.35 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.17 { \scriptstyle \,\pm\, 1.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}2.70 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}2.60 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}2.82 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ & - & $\text{--}0.03 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $\text{--}0.48 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}0.79 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.48 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}1.04 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ & $2.47 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}1.91 { \scriptstyle \,\pm\, 0.03 }$ & $\text{--}1.48 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.85 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.66 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.30 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}13.7 { \scriptstyle \,\pm\, 0.82 }$ & $\text{--}3.96 { \scriptstyle \,\pm\, 0.04 }$ & $\text{--}3.80 { \scriptstyle \,\pm\, 0.02 }$ & - & $\text{--}4.98 { \scriptstyle \,\pm\, 0.02 }$ \\
\midrule\multicolumn{7}{l}{\textsc{Extrapolation beyond training range}} \\[0.5em] 
GP (full) & &
    $4.29 { \scriptstyle \,\pm\, 6.2\text{\textsc{e}}{\,\text{--}3} }$ &
    $0.82 { \scriptstyle \,\pm\, 4.3\text{\textsc{e}}{\,\text{--}3} }$ &
    $0.66 { \scriptstyle \,\pm\, 2.2\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}0.33 { \scriptstyle \,\pm\, 3.4\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
GP (diag) & &
    $\text{--}1.40 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}1.41 { \scriptstyle \,\pm\, 4.8\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}1.72 { \scriptstyle \,\pm\, 6.2\text{\textsc{e}}{\,\text{--}3} }$ &
    $\text{--}1.40 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ &
    N/A \\
ConvCNP & & $\text{--}1.41 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.41 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.73 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.41 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $0.27 { \scriptstyle \,\pm\, 0.02 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{ML}}$ & $\text{--}1.09 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.11 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.30 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.24 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $1.61 { \scriptstyle \,\pm\, 0.02 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}1.29 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.29 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.55 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.34 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.25 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}2.23 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}2.08 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}2.50 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.39 { \scriptstyle \,\pm\, 4.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.06 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $\text{--}1.21 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.31 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.19 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.51 { \scriptstyle \,\pm\, 8.0\text{\textsc{e}}{\,\text{--}3} }$ & $2.10 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}1.44 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.45 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.77 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.46 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}0.20 { \scriptstyle \,\pm\, 2.0\text{\textsc{e}}{\,\text{--}3} }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}5.85 { \scriptstyle \,\pm\, 0.05 }$ & $\text{--}2.65 { \scriptstyle \,\pm\, 3.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}4.06 { \scriptstyle \,\pm\, 0.04 }$ & $\text{--}1.49 { \scriptstyle \,\pm\, 5.0\text{\textsc{e}}{\,\text{--}3} }$ & $\text{--}1.99 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ \\
\bottomrule

\end{tabular}
\end{center}
\end{table}


==> arxiv_camera_ready_full copy/tables/bakeoff1d_fixed.tex <==
\begin{table}
\footnotesize
\caption{Log-likelihood for ConvCNP, ConvNP, ANP, and NP. Each of the stochastic models was trained on each dataset with $\gL_{\mathrm{ML}}$, $\gL_{\mathrm{IW}}$, and $\gL_{\mathrm{NP}}$, separately. The noise model for these experiments was a fixed constant, shared across all stochastic models.}
\label{table:1d_bakeoff_fixed}
\begin{center}
\begin{tabular}{l@{\hspace{4pt}}l@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}

\toprule 
 & & \multicolumn{1}{c}{EQ} & \multicolumn{1}{c}{Mat\'ern--$\frac52$} & \multicolumn{1}{c}{Noisy Mixt.} & \multicolumn{1}{c}{Weakly Per.} & \multicolumn{1}{c}{Sawtooth}\\
\midrule\multicolumn{7}{l}{\textsc{Interpolation inside training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $\text{--}29.0 { \scriptstyle \,\pm\, 0.78 }$ & $\text{--}39.6 { \scriptstyle \,\pm\, 0.86 }$ & $\text{--}38.8 { \scriptstyle \,\pm\, 1.14 }$ & $\text{--}67.6 { \scriptstyle \,\pm\, 0.93 }$ & $0.53 { \scriptstyle \,\pm\, 0.03 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}42.1 { \scriptstyle \,\pm\, 1.11 }$ & $\text{--}49.7 { \scriptstyle \,\pm\, 1.03 }$ & $\text{--}49.8 { \scriptstyle \,\pm\, 1.38 }$ & $\text{--}107 { \scriptstyle \,\pm\, 1.23 }$ & $\text{--}8.71 { \scriptstyle \,\pm\, 0.07 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}45.4 { \scriptstyle \,\pm\, 0.97 }$ & $\text{--}54.7 { \scriptstyle \,\pm\, 0.92 }$ & $\text{--}61.6 { \scriptstyle \,\pm\, 1.31 }$ & $\text{--}108 { \scriptstyle \,\pm\, 1.25 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $\text{--}0.32 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.02 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.98 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}2.05 { \scriptstyle \,\pm\, 0.01 }$ & $1.05 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}12.1 { \scriptstyle \,\pm\, 0.39 }$ & $\text{--}17.8 { \scriptstyle \,\pm\, 0.42 }$ & $\text{--}15.4 { \scriptstyle \,\pm\, 0.46 }$ & $\text{--}57.4 { \scriptstyle \,\pm\, 0.76 }$ & $\text{--}6.85 { \scriptstyle \,\pm\, 0.09 }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{--}7.05 { \scriptstyle \,\pm\, 0.12 }$ & $\text{--}12.5 { \scriptstyle \,\pm\, 0.17 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.16 }$ & $\text{--}79.0 { \scriptstyle \,\pm\, 0.97 }$ & $\text{--}9.47 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $\text{--}1.21 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}3.50 { \scriptstyle \,\pm\, 0.04 }$ & $\text{--}2.68 { \scriptstyle \,\pm\, 0.05 }$ & $\text{--}2.14 { \scriptstyle \,\pm\, 0.01 }$ & $1.11 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}14.9 { \scriptstyle \,\pm\, 0.43 }$ & $\text{--}25.0 { \scriptstyle \,\pm\, 0.54 }$ & $\text{--}26.7 { \scriptstyle \,\pm\, 0.60 }$ & $\text{--}82.9 { \scriptstyle \,\pm\, 1.04 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.09 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}9.62 { \scriptstyle \,\pm\, 0.17 }$ & $\text{--}15.6 { \scriptstyle \,\pm\, 0.24 }$ & $\text{--}14.0 { \scriptstyle \,\pm\, 0.26 }$ & $\text{--}89.7 { \scriptstyle \,\pm\, 1.09 }$ & $\text{--}13.1 { \scriptstyle \,\pm\, 0.06 }$ \\
\midrule\multicolumn{7}{l}{\textsc{Interpolation beyond training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}115 { \scriptstyle \,\pm\, 1.85 }$ & $\text{--}117 { \scriptstyle \,\pm\, 1.73 }$ & $\text{--}156 { \scriptstyle \,\pm\, 2.80 }$ & $\text{--}143 { \scriptstyle \,\pm\, 1.62 }$ & $\text{--}14.2 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}114 { \scriptstyle \,\pm\, 2.41 }$ & $\text{--}118 { \scriptstyle \,\pm\, 1.64 }$ & $\text{--}138 { \scriptstyle \,\pm\, 2.40 }$ & $\text{--}131 { \scriptstyle \,\pm\, 1.48 }$ & $\text{--}14.8 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}323 { \scriptstyle \,\pm\, 18.0 }$ & $\text{--}387 { \scriptstyle \,\pm\, 23.4 }$ & $\text{--}240 { \scriptstyle \,\pm\, 8.83 }$ & $\text{--}881 { \scriptstyle \,\pm\, 63.8 }$ & $\text{--}1.01\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 1.64\text{\textsc{e}}{4} }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{{NaN}} { \scriptstyle \,\pm\, \text{{NaN}} }$ & $\text{{NaN}} { \scriptstyle \,\pm\, \text{{NaN}} }$ & $\text{--}9.34\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 1.55\text{\textsc{e}}{3} }$ & $\text{--}3.71\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 313 }$ & $\text{--}7.18\text{\textsc{e}}{5} { \scriptstyle \,\pm\, 9.19\text{\textsc{e}}{5} }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}1.02\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 84.3 }$ & $\text{--}6.96\text{\textsc{e}}{5} { \scriptstyle \,\pm\, 1.03\text{\textsc{e}}{6} }$ & $\text{--}552 { \scriptstyle \,\pm\, 35.3 }$ & $\text{--}973 { \scriptstyle \,\pm\, 72.4 }$ & $\text{--}14.4 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}5.91\text{\textsc{e}}{7} { \scriptstyle \,\pm\, 3.95\text{\textsc{e}}{7} }$ & $\text{--}8.07\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 5.31\text{\textsc{e}}{4} }$ & $\text{--}2.93\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 1.08\text{\textsc{e}}{4} }$ & $\text{--}8.56\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 3.24\text{\textsc{e}}{4} }$ & $\text{--}1.12\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 6.10\text{\textsc{e}}{3} }$ \\
\midrule\multicolumn{7}{l}{\textsc{Extrapolation beyond training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}120 { \scriptstyle \,\pm\, 1.87 }$ & $\text{--}119 { \scriptstyle \,\pm\, 1.73 }$ & $\text{--}138 { \scriptstyle \,\pm\, 2.36 }$ & $\text{--}131 { \scriptstyle \,\pm\, 1.43 }$ & $\text{--}14.0 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}194 { \scriptstyle \,\pm\, 4.68 }$ & $\text{--}164 { \scriptstyle \,\pm\, 3.32 }$ & $\text{--}173 { \scriptstyle \,\pm\, 4.01 }$ & $\text{--}132 { \scriptstyle \,\pm\, 1.56 }$ & $\text{--}14.1 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}567 { \scriptstyle \,\pm\, 6.18 }$ & $\text{--}691 { \scriptstyle \,\pm\, 8.56 }$ & $\text{--}567 { \scriptstyle \,\pm\, 7.17 }$ & $\text{--}1.48\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 36.4 }$ & $\text{--}540 { \scriptstyle \,\pm\, 5.93 }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{--}2.19\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 51.9 }$ & $\text{--}704 { \scriptstyle \,\pm\, 11.4 }$ & $\text{--}4.00\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 113 }$ & $\text{--}3.64\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 105 }$ & $\text{--}54.8 { \scriptstyle \,\pm\, 0.46 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}2.52\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 60.7 }$ & $\text{--}8.59\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 256 }$ & $\text{--}1.43\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 42.2 }$ & $\text{--}1.11\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 36.3 }$ & $\text{--}14.1 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}6.75\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 266 }$ & $\text{--}1.93\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 702 }$ & $\text{--}1.12\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 41.4 }$ & $\text{--}1.04\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 440 }$ & $\text{--}1.58\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 30.9 }$ \\
\bottomrule

\end{tabular}
\end{center}
\end{table}


==> arxiv_camera_ready_full copy/tables/bakeoff_main_text.tex <==
\begin{table}[t]
\footnotesize
\caption{Log-likelihood of ConvNP and ANP trained with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$ on 1D regression tasks.}
\label{table:1d_bakeoff_main_text}
\begin{center}
\begin{tabular}{@{}l@{\hspace{4pt}}
                c@{\hspace{4pt}}
                c@{\hspace{6pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{}}

\toprule 
 & & &
 \multicolumn{3}{c}{\textsc{within training range}} & 
 \multicolumn{3}{c}{\textsc{beyond training range}}\\
 \midrule
 & \textsc{train} & \textsc{eval} &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  & 
 \multicolumn{1}{c}{Weakly Per.}         & 
 \multicolumn{1}{c}{Sawtooth}            &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  &
 \multicolumn{1}{c}{Weakly Per.}         &
 \multicolumn{1}{c}{Sawtooth}\\
 \midrule
 %
 ConvNP & $\gL_{\mathrm{ML}}$ & ML & 
 $\textbf{\text{--}0.80} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$ &         %   Matern Interpolation
 $\textbf{\text{--}1.08} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Interpolation 
 $\textbf{1.22} { \scriptstyle \,\pm\, 0.01 }$                                               &         %   Sawtooth Interpolation 
 $\textbf{\text{--}0.80} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$ &         %   Matern Extrapolation
 $\textbf{\text{--}1.08} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Extrapolation 
 $\textbf{1.23} { \scriptstyle \,\pm\, 0.01 }$ \\                    %   Sawtooth Extrapolation 
 %
 ANP & $\gL_{\mathrm{ML}}$ & ML & 
 $\text{--}0.90 { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Interpolation
 $\text{--}1.20 { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $\text{--}0.03 { \scriptstyle \,\pm\, 3\text{\textsc{e}}{\,\text{--}3} }$ &        %   Sawtooth Interpolation
 $\text{--}1.30 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Extrapolation
 $\text{--}1.34 { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Extrapolation
 $\text{--}0.20 { \scriptstyle \,\pm\, 2\text{\textsc{e}}{\,\text{--}3} }$ \\ %   Sawtooth Extrapolation
 %
 \midrule
 %
 ConvNP & $\gL_{\mathrm{NP}}$ & IW &
 $\textbf{\text{--}0.89} { \scriptstyle \,\pm\, 0.01 }$          &     %   Matern Interpolation
 $\textbf{\text{--}1.11} { \scriptstyle \,\pm\, 0.01 }$ &     %   Weakly Per.
 $\textbf{1.53} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$          &     %   Sawtooth Interpolation
 $\textbf{\text{--}0.89} { \scriptstyle \,\pm\, 0.03 }$          &     %   Matern Extrapolation
 $\textbf{\text{--}1.10} { \scriptstyle \,\pm\, 0.01 }$ &     %   Weakly Per. Extrapolation
 $\textbf{1.52} { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 ANP & $\gL_{\mathrm{NP}}$ & IW &
 $\text{--}0.95 { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Interpolation
 $\text{--}1.18 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $\text{--}0.02 { \scriptstyle \,\pm\, 4\text{\textsc{e}}{\,\text{--}3} }$ &        %   Sawtooth Interpolation
 $\text{--}4.09 { \scriptstyle \,\pm\, 0.18 }$                             &        %   Matern Extrapolation
 $\text{--}1.60 { \scriptstyle \,\pm\, 0.02 }$                             &        %   Weakly Per. Extrapolation
 $\text{--}0.19 { \scriptstyle \,\pm\, 2\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 \midrule
 %
  ConvCNP & & &
 $\text{--}{0.88} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Interpolation
 $\text{--}{1.18} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$                                    &         %   Weakly Per. Interpolation 
 $1.15 { \scriptstyle \,\pm\, 0.05 }$                                               &         %   Sawtooth Interpolation 
 $\text{--}{0.88} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Extrapolation
 $\text{--}{1.18} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$                                    &         %   Weakly Per. Extrapolation 
 $1.14 { \scriptstyle \,\pm\, 0.04 }$ \\                    %   Sawtooth Extrapolation 
 %
 \bottomrule

\end{tabular}
\end{center}
\end{table}


==> arxiv_camera_ready_full copy/tables/environmental_metrics.tex <==
\begin{table}[htb] 
\vspace*{-0.5em}
\caption{Average joint predictive log-likelihood (LL) and RMSE on ERA5Land. }
\label{table:era5_loglik_rmse}
\begin{center}
\begin{tabular}{
    l@{\hspace{4pt}}
    l@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}c}
\toprule 
 & &
 \multicolumn{1}{r}{Central (train)} & 
 \multicolumn{1}{r}{West (test)} & 
 \multicolumn{1}{r}{East (test)} & 
 \multicolumn{1}{r}{South (test)}\\
 %
 \midrule 
 %
 LL &  ConvNP  & 
 $\textbf{6.16} { \scriptstyle \,\pm\, 0.098 }$ & 
 $\textbf{5.87} { \scriptstyle \,\pm\, 0.104 }$ & 
 $\textbf{6.78} { \scriptstyle \,\pm\, 0.106 }$ & 
 $\textbf{8.51} { \scriptstyle \,\pm\, 0.169 }$ \\
 %
 & GP & 
 $4.95 { \scriptstyle \,\pm\, 0.072 }$ & 
 $4.89 { \scriptstyle \,\pm\, 0.087 }$ & 
 $5.31 { \scriptstyle \,\pm\, 0.100 }$ & 
 $6.23 { \scriptstyle \,\pm\, 0.109 }$ \\[.5em]
 %
 RMSE & ConvNP & 
 $\textbf{2.13}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.34\text{\textsc{e}}{-4} }$ &
 $\textbf{2.62}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 3.55\text{\textsc{e}}{-4} }$ & 
 $\textbf{1.18}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.32\text{\textsc{e}}{-4} }$ & 
 $6.79\text{\textsc{e}}{-4} { \scriptstyle \,\pm\, 8.14\text{\textsc{e}}{-5} }$ \\
 %
  & GP & 
 $2.50\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.59\text{\textsc{e}}{-4} }$ & 
 $\textbf{2.21}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.34\text{\textsc{e}}{-4} }$ & 
 $\textbf{1.13}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 4.60\text{\textsc{e}}{-5} }$ &
 $\textbf{4.10}\text{\textsc{e}}{-4} { \scriptstyle \,\pm\, 3.49\text{\textsc{e}}{-5} }$ \\
 \bottomrule
\end{tabular}
\end{center}
\end{table}

==> arxiv_camera_ready_full copy/tables/environmental_metrics_v2.tex <==
\begin{table}[t] 
\footnotesize
\caption{
    Joint predictive log-likelihoods (LL) and RMSEs on ERA5-Land, averaged over 1000 tasks.
    %Results within standard error of best result in bold.
}
\label{table:era5_loglik_rmse}
\begin{center}
\begin{tabular}{@{}llcccc@{}}
\toprule
&        & 
    Central (train) & 
    West (test)     & 
    East (test)     & 
    South (test)   \\ 
    \midrule
    \multirow{2}{*}{LL}   & 
    ConvNP                & 
    $\textbf{4.47} { \scriptstyle \,\pm\, 0.07 }$  & 
    $\textbf{4.55} { \scriptstyle \,\pm\, 0.08 }$  & 
    $\textbf{5.07} { \scriptstyle \,\pm\, 0.07 }$  & 
    $\textbf{4.65} { \scriptstyle \,\pm\, 0.08 }$   \\
    & GP     & 
    $3.33 { \scriptstyle \,\pm\, 0.06 }$           & 
    $3.65 { \scriptstyle \,\pm\, 0.06 }$           & 
    $4.07 { \scriptstyle \,\pm\, 0.06 }$           & 
    $3.34 { \scriptstyle \,\pm\, 0.06}$ \\
    \multirow{2}{*}{RMSE ($\times 10^{-2}$)}                           & 
    ConvNP                                          & 
    $\textbf{5.72} { \scriptstyle \,\pm\, 0.33 }$ & 
    $\textbf{5.77} { \scriptstyle \,\pm\, 0.37 }$ & 
    $\textbf{3.23} { \scriptstyle \,\pm\, 0.22 }$ & 
    $\textbf{6.92} { \scriptstyle \,\pm\, 0.39 }$          \\
    & GP     & 
    $\textbf{6.26} { \scriptstyle \,\pm\, 0.30 }$          & 
    $\textbf{5.75} { \scriptstyle \,\pm\, 0.29 }$ & 
    $\textbf{3.10} { \scriptstyle \,\pm\, 0.18 }$ & 
    $7.94 { \scriptstyle \,\pm\, 0.44 }$ \\ 
    \bottomrule
\end{tabular}
\end{center}
\end{table}

==> arxiv_camera_ready_full copy/tables/gp1d_table.tex <==
\begin{table}[t]
\footnotesize
\caption{Log-likelihoods on 1D regression tasks. Lower bounds marked with asterisk. Highest non-GP values in bold.}
\label{table:1d_bakeoff_main_text}
\begin{center}
\begin{tabular}{@{}l@{\hspace{4pt}}
                c@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{}}

\toprule 
 & &
 \multicolumn{3}{c}{\textsc{within training range}} & 
 \multicolumn{3}{c}{\textsc{beyond training range}}\\
 \midrule
 &  &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  & 
 \multicolumn{1}{c}{Weakly Per.}         & 
 \multicolumn{1}{c}{Sawtooth}            &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  &
 \multicolumn{1}{c}{Weakly Per.}         &
 \multicolumn{1}{c}{Sawtooth}\\[0.2em]
 %
 GP  & (full) &
 $1.22 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$             &         %   Matern Interpolation
 $\text{--}{0.06} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$  &         %   Weakly Per. Interpolation 
 \multicolumn{1}{c}{N/A}                                                      &         %   Sawtooth Interpolation 
 $1.22 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$             &         %   Matern Extrapolation
 $\text{--}{0.06} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$  &         %   Weakly Per. Extrapolation 
 \multicolumn{1}{c}{N/A}      \\                                                        %   Sawtooth Extrapolation 
 %
 ConvNP$^\ast$ & ($\gL_{\mathrm{ML}}$) & 
 $\text{--}\textbf{0.58} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   Matern Interpolation
 $\text{--}\textbf{1.02} { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Interpolation 
 $\textbf{2.30} { \scriptstyle \,\pm\, 0.01 }$                                      &         %   Sawtooth Interpolation 
 $\text{--}\textbf{0.58} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   Matern Extrapolation
 $\text{--}\textbf{1.03} { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Extrapolation 
 $\textbf{2.29} { \scriptstyle \,\pm\, 0.02 }$ \\                                             %   Sawtooth Extrapolation 
 %
 ANP$^\ast$ & ($\gL_{\mathrm{ML}}$) & 
 $\text{--}0.73 { \scriptstyle \,\pm\, 0.01 }$ &                                    %   Matern Interpolation
 $\text{--}1.14 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $0.09 { \scriptstyle \,\pm\, 3\text{\textsc{e}}{\,\text{--}3} }$ &                 %   Sawtooth Interpolation
 $\text{--}1.39 { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Extrapolation
 $\text{--}1.35 { \scriptstyle \,\pm\, 4\text{\textsc{e}}{\,\text{--}3} }$                             &        %   Weakly Per. Extrapolation
 $\text{--}0.17 { \scriptstyle \,\pm\, 1\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 ANP$^\ast$ & ($\gL_{\mathrm{NP}}$) & 
 $\text{--}0.96 { \scriptstyle \,\pm\, 0.01 }$ &                                    %   Matern Interpolation
 $\text{--}1.37 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $0.20 { \scriptstyle \,\pm\, 9\text{\textsc{e}}{\,\text{--}3} }$ &                 %   Sawtooth Interpolation
 $\text{--}1.48 { \scriptstyle \,\pm\, 4\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Extrapolation
 $\text{--}1.66 { \scriptstyle \,\pm\, 0.01 }$                             &        %   Weakly Per. Extrapolation
 $\text{--}0.30 { \scriptstyle \,\pm\, 4\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 GP  & (diag) &
 $\text{--}{0.84} { \scriptstyle \,\pm\, 9\text{\textsc{e}}{\,\text{--}3} }$        &         %   Matern Interpolation
 $\text{--}{1.17} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$        &         %   Weakly Per. Interpolation 
 \multicolumn{1}{c}{N/A}                                                            &         %   Sawtooth Interpolation 
 $\text{--}{0.84} { \scriptstyle \,\pm\, 9\text{\textsc{e}}{\,\text{--}3} }$        &         %   Matern Extrapolation
 $\text{--}{1.17} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$        &         %   Weakly Per. Extrapolation 
 \multicolumn{1}{c}{N/A}   \\                                                                 %   Sawtooth Extrapolation 
 %
 ConvCNP & &
 $\text{--}{0.88} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Interpolation
 $\text{--}{1.19} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$        &         %   Weakly Per. Interpolation 
 $1.15 { \scriptstyle \,\pm\, 0.04 }$                                               &         %   Sawtooth Interpolation 
 $\text{--}{0.87} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Extrapolation
 $\text{--}{1.19} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$        &         %   Weakly Per. Extrapolation 
 $1.11 { \scriptstyle \,\pm\, 0.04 }$ \\                                                      %   Sawtooth Extrapolation 
 %
 \bottomrule

\end{tabular}
\end{center}
\vspace*{-2em}
\end{table}


==> arxiv_camera_ready_full copy/tables/image_main_text_squeeze_hetero.tex <==
\begin{table}[t]
\footnotesize
\caption{Test log-likelihood lower bounds for image completion (5 runs).}
\label{table:images_main_text}
\vspace*{-2pt}
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{} & 
\multicolumn{2}{c}{MNIST}                 & 
\multicolumn{2}{c}{CelebA32}              & 
\multicolumn{2}{c}{SVHN}                  & 
\multicolumn{2}{c}{ZSMM}                  \\ 
%
& 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ & $\gL_{\mathrm{NP}}$ \\ 
%
\midrule
%
ConvNP    &  
$1.28 { \scriptstyle \,\pm\, 0.00 }$  &   % MNIST ML
$1.16 { \scriptstyle \,\pm\, 0.16 }$           &   % MNIST NP                 
$\textbf{6.92} { \scriptstyle \,\pm\, 0.10 }$  &   % CELEBA ML              
$-0.27 { \scriptstyle \,\pm\, 0.00 }$           &   % CELEBA NP
$\textbf{9.89} { \scriptstyle \,\pm\, 0.09}$   &   % SVHN ML                   
$0.17 { \scriptstyle \,\pm\, 0.00 }$           &   % SVHN NP                   
$\textbf{3.75} { \scriptstyle \,\pm\, 0.01 }$  &   % ZSMM ML
$0.13  { \scriptstyle \,\pm\, 0.00}$           \\  % ZSMM NP
%
ANP   &
$1.26 { \scriptstyle \,\pm\, 0.00 }$           &  % MNIST ML
$\textbf{1.29} { \scriptstyle \,\pm\, 0.00 }$           &  % MNIST NP           
$5.98 { \scriptstyle \,\pm\, 0.08 }$           &  % CELEBA ML         
$6.04 { \scriptstyle \,\pm\, 0.10 }$           &  % CELEBA NP         
$9.18 { \scriptstyle \,\pm\, 0.08 }$           &  % SVHN ML         
$8.91 { \scriptstyle \,\pm\, 0.06 }$           &  % SVHN NP         
$-2.03 { \scriptstyle \,\pm\, 0.08 }$           &  % ZSMM ML         
$-2.13 { \scriptstyle \,\pm\, 0.27 }$           \\ % ZSMM NP
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\vspace*{-1.0em}
\end{table}

% NOTE : here all the models are heteroskedastic

==> arxiv_camera_ready_full copy/tables/image_main_text_squeezed_homo.tex <==
\begin{table}[t]
\footnotesize
\caption{Test log-likelihood lower bounds for image completion (5 runs).}
\label{table:images_main_text}
\vspace*{-2pt}
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{} & 
\multicolumn{2}{c}{MNIST}                 & 
\multicolumn{2}{c}{CelebA32}              & 
\multicolumn{2}{c}{SVHN}                  & 
\multicolumn{2}{c}{ZSMM}                  \\ 
%
& 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ & $\gL_{\mathrm{NP}}$ \\ 
%
\midrule
%
ConvNP    &  
$\textbf{2.11} { \scriptstyle \,\pm\, 0.01 }$  &   % MNIST ML
$0.99 { \scriptstyle \,\pm\, 0.42 }$           &   % MNIST NP                 
$\textbf{6.92} { \scriptstyle \,\pm\, 0.10 }$  &   % CELEBA ML              
$-0.27 { \scriptstyle \,\pm\, 0.00 }$           &   % CELEBA NP
$\textbf{9.89} { \scriptstyle \,\pm\, 0.09}$   &   % SVHN ML                   
$0.17 { \scriptstyle \,\pm\, 0.00 }$           &   % SVHN NP                   
$\textbf{4.58} { \scriptstyle \,\pm\, 0.04 }$  &   % ZSMM ML
$0.14  { \scriptstyle \,\pm\, 0.00}$           \\  % ZSMM NP
%
ANP   &
$1.66 { \scriptstyle \,\pm\, 0.03 }$           &  % MNIST ML
$1.64 { \scriptstyle \,\pm\, 0.03 }$           &  % MNIST NP           
$5.98 { \scriptstyle \,\pm\, 0.08 }$           &  % CELEBA ML         
$6.04 { \scriptstyle \,\pm\, 0.10 }$           &  % CELEBA NP         
$9.18 { \scriptstyle \,\pm\, 0.08 }$           &  % SVHN ML         
$8.91 { \scriptstyle \,\pm\, 0.06 }$           &  % SVHN NP         
$-10.8 { \scriptstyle \,\pm\, 1.99 }$           &  % ZSMM ML         
$-6.45 { \scriptstyle \,\pm\, 0.99 }$           \\ % ZSMM NP
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\vspace*{-1.0em}
\end{table}

% Note : MNIST and ZSMM is homoskedastic  the rest is hetero

==> arxiv_camera_ready_full copy/tables/images_main_text.tex <==
\begin{table}[htb]
\begin{center}
\caption{Per-pixel test log-likelihood of ConvNP and ANP trained with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$ (5 runs).}
\label{table:images_main_text}
\begin{tabular}{l@{\hspace{4pt}}
                l@{\hspace{6pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{0pt}}}

\toprule 
 & & 
 \multicolumn{1}{c}{MNIST} & 
 \multicolumn{1}{c}{CelebA32}         & 
 \multicolumn{1}{c}{SVHN}           &
 \multicolumn{1}{c}{ZSMM}           \\
 \midrule
 %
 ConvNP & $\gL_{\mathrm{ML}}$ & 
 $\textbf{2.03} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   MNIST
 $\textbf{4.11} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   CELEBA
 $\textbf{8.35} { \scriptstyle \,\pm\, 0.05}$ &         %   SVHN
 $\textbf{1.39} { \scriptstyle \,\pm\, 0.03 }$ \\[.2em]                                    %   ZSMM
 %
 ConvNP & $\gL_{\mathrm{NP}}$ &
 $1.02 { \scriptstyle \,\pm\, 0.00 }$ &     %   MNIST
 $2.13 { \scriptstyle \,\pm\, 0.12  }$ &     %   CELEBA
 $4.71 { \scriptstyle \,\pm\, 0.02 }$          &     %   SVHN
 $0.04  { \scriptstyle \,\pm\, 0.00}$ \\[.2em]      %   ZSMM
 %
 ANP & $\gL_{\mathrm{ML}}$ & 
 $1.82 { \scriptstyle \,\pm\, 0.01 }$ &                                    %   MNIST
 $3.72 { \scriptstyle \,\pm\, 0.02 }$ &                                             %   CELEBA
 $7.71 { \scriptstyle \,\pm\, 0.03 }$          &        %   SVHN
 $0.42 { \scriptstyle \,\pm\, 0.03 }$  \\[.2em]        %   ZSMM 
 %
 ANP & $\gL_{\mathrm{NP}}$ &
 $1.05 { \scriptstyle \,\pm\, 0.07 }$ &                                    %   MNIST
 $3.57 { \scriptstyle \,\pm\, 0.02 }$ &        %   CELEBA
 $7.62 { \scriptstyle \,\pm\,  0.05}$          &        %   SVHN
 $0.24 { \scriptstyle \,\pm\, 0.04 }$ \\         %   ZSMM
 \bottomrule

\end{tabular}
\end{center}
\end{table}


==> arxiv_camera_ready_full copy/tables/parameter_counts_1d.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{rccccc}
        \toprule
        & EQ & Mat\'ern--$\frac52$ & Noisy Mixt.\ & Weakly Per.\ & Sawtooth \\ \midrule
        ConvCNP & $42\,822$ & $42\,822$ & $51\,014$ & $51\,014$ & $100\,166$ \\
        ConvNP & $88\,486$ & $88\,486$ & $104\,870$ & $104\,870$ & $203\,174$ \\
        ANP & $530\,178$ & $530\,178$ & $530\,178$ & $530\,178$ & $530\,178$ \\
        NP & $479\,874$ & $479\,874$ & $479\,874$ & $479\,874$ & $479\,874$ \\
        \bottomrule
    \end{tabular}
    \vspace*{5pt}
    \caption{Parameter counts for the ConvCNP, ConvNP, ANP, and NP in the 1D regression tasks}
    \label{tab:1D_parameter_counts}
\end{table}

==> arxiv_camera_ready_full copy/tables/region_coordinates.tex <==
% Central Europe (8, 28) (52, 46) 
% West box (1, 8) (50, 46)
% East box (28,35) (52, 49)
% South box (19, 26) (46, 42)

\begin{table}[htb] 
\caption{Coordinates for boxes defining the train and test regions. Latitidues are given as (north, south), and longitudes as (west, east).}
\label{table:era5_region_coordinates}
\begin{center}
\begin{tabular}{l@{\hspace{4pt}}
c@{\hspace{4pt}}
c@{\hspace{4pt}}
c@{\hspace{4pt}}
c@{\hspace{4pt}}}
\toprule 
 & 
 \multicolumn{1}{c}{Central (train)} & 
 \multicolumn{1}{c}{Western (test)} & 
 \multicolumn{1}{c}{Eastern (test)} & 
 \multicolumn{1}{c}{Southern (test)}\\
 %
 \midrule 
 %
 Latitudes  & 
 $(52, 46)$ & 
 $(50, 46)$ & 
 $(52, 49)$ & 
 $(46, 42)$ \\
 %
 Longitudes & 
 $(08, 28)$ & 
 $(01, 08)$ & 
 $(28, 35)$ & 
 $(19, 26)$ \\
 %
 \bottomrule
\end{tabular}
\end{center}
\end{table}

==> diagrams/forward_pass.tex <==
% Source: https://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,color=white,fill=black,draw,inner sep=1pt] (char) {#1};}}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{plots/gp1d/forward_pass.pdf}%
    \begin{tikzpicture}[overlay, remember picture]
        \node [anchor=south] () at (-11.8cm, 2cm) {\scriptsize \circled{\textbf{1}}\hspace{5 pt}Context set $D_c$};
        \node [anchor=south] () at (-7cm, 2cm) {\scriptsize \circled{\textbf{2}}\hspace{5 pt}Encoder: $z \sim \mathrm{ConvCNP}(D_c)$};
        \node [anchor=south] () at (-2cm, 2cm) {\scriptsize \circled{\textbf{3}}\hspace{5 pt}Decoder: $f = d(z)$};
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-9.6cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{E}_\vphi$
        } (-9.25cm, 0.9cm);
        \draw [
            line width=1mm,
            ->,
            > = {
                Triangle[length=1mm, width=2.0mm]
            }
        ] (-4.7cm, 0.9cm) -- node [pos=0.5, anchor=south] {
            \footnotesize
            $\mathrm{D}_\vtheta$
        } (-4.35cm, 0.9cm);
    \end{tikzpicture}%
    \caption{
        Encoder-decoder architecture. The ConvCNP encoder takes the context set as input (left panel) and outputs a single sample of $z$ (center panel). The decoder takes this as input and outputs a predictive sample (right panel blue; two other samples shown in grey).
    }
    \label{fig:forward_pass}
    %\vspace*{-1.5em}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> plots/image_completion/image_figures_hetero.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}[b]{0.43\textwidth}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_convnp_hetero.png}
        \subcaption{ConvNP}
        \label{fig:images_zsmm_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_anp_hetero.png}
        \subcaption{ANP}
        \label{fig:images_zsmm_anp}
    \end{subfigure}
    %
\end{subfigure}
%
\begin{subfigure}[b]{0.56\textwidth}
%
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp_hetero.png}
        \subcaption{ConvNP}
        \label{fig:images_marginal_convnp}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_anp_hetero.png}
        \subcaption{ANP}
        \label{fig:images_marginal_anp}
    \end{subfigure}
%
\end{subfigure}
%
\caption{Left two plots: predictive samples on zero-shot multi MNIST. Right two plots: samples and marginal predictives on standard MNIST. We plot the density of the five marginals that maximize Sarle's bimodality coefficient \cite{ellison1987effect}. We use $\gL_{\mathrm{ML}}$ for training.
Blue pixels are not in the context set.}
\label{fig:images_zsmm}
%\vspace*{-1.5em}
\end{figure}

==> plots/image_completion/marginal/marginal_pred.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}{0.49\columnwidth}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp.png}
%\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_convnp.png}
\end{subfigure}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_convnp.png}
\end{subfigure} 
\subcaption{ConvNP}
\label{fig:images_marginal_convnp}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_anp.png}
%\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_five_anp.png}
\end{subfigure}
\begin{subfigure}{0.47\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/marginal/marginal_pred_top_anp.png}
\end{subfigure}
\subcaption{ANP}
\label{fig:images_marginal_anp}
\end{subfigure}
\caption{Samples and associated marginal predictives from (a) ConvNP and (b) ANP. 
We selected marginal predictive that were multi-modal by considering the seven ones that maximize Sarle's bimodality coefficient \cite{ellison1987effect}. Blue pixels correspond to the ones that are not in the context set. 
}
\label{fig:images_marginal_pred}
\end{figure}

==> plots/image_completion/zsmm/zsmm.tex <==
\begin{figure}[t]
    \centering
\begin{subfigure}{0.27\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_convnp.png}
\subcaption{ConvNP}
\label{fig:images_zsmm_convnp}
\end{subfigure}
\begin{subfigure}{0.27\columnwidth}
\includegraphics[width=\textwidth]{plots/image_completion/zsmm/zsmms_anp.png}
\subcaption{ANP}
\label{fig:images_zsmm_anp}
\end{subfigure}
\caption{Samples from the ANP and ConvNP in a zero-shot spatial generalization task, where the models are trained on single digits and tested on multiple digits. 
}
\label{fig:images_zsmm}
\end{figure}

==> tables/bakeoff1d_fixed.tex <==
\begin{table}
\footnotesize
\caption{Log-likelihood for ConvCNP, ConvNP, ANP, and NP. Each of the stochastic models was trained on each dataset with $\gL_{\mathrm{ML}}$, $\gL_{\mathrm{IW}}$, and $\gL_{\mathrm{NP}}$, separately. The noise model for these experiments was a fixed constant, shared across all stochastic models.}
\label{table:1d_bakeoff_fixed}
\begin{center}
\begin{tabular}{l@{\hspace{4pt}}l@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}

\toprule 
 & & \multicolumn{1}{c}{EQ} & \multicolumn{1}{c}{Mat\'ern--$\frac52$} & \multicolumn{1}{c}{Noisy Mixt.} & \multicolumn{1}{c}{Weakly Per.} & \multicolumn{1}{c}{Sawtooth}\\
\midrule\multicolumn{7}{l}{\textsc{Interpolation inside training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $\text{--}29.0 { \scriptstyle \,\pm\, 0.78 }$ & $\text{--}39.6 { \scriptstyle \,\pm\, 0.86 }$ & $\text{--}38.8 { \scriptstyle \,\pm\, 1.14 }$ & $\text{--}67.6 { \scriptstyle \,\pm\, 0.93 }$ & $0.53 { \scriptstyle \,\pm\, 0.03 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}42.1 { \scriptstyle \,\pm\, 1.11 }$ & $\text{--}49.7 { \scriptstyle \,\pm\, 1.03 }$ & $\text{--}49.8 { \scriptstyle \,\pm\, 1.38 }$ & $\text{--}107 { \scriptstyle \,\pm\, 1.23 }$ & $\text{--}8.71 { \scriptstyle \,\pm\, 0.07 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}45.4 { \scriptstyle \,\pm\, 0.97 }$ & $\text{--}54.7 { \scriptstyle \,\pm\, 0.92 }$ & $\text{--}61.6 { \scriptstyle \,\pm\, 1.31 }$ & $\text{--}108 { \scriptstyle \,\pm\, 1.25 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $\text{--}0.32 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}1.02 { \scriptstyle \,\pm\, 0.01 }$ & $\text{--}0.98 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}2.05 { \scriptstyle \,\pm\, 0.01 }$ & $1.05 { \scriptstyle \,\pm\, 7.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}12.1 { \scriptstyle \,\pm\, 0.39 }$ & $\text{--}17.8 { \scriptstyle \,\pm\, 0.42 }$ & $\text{--}15.4 { \scriptstyle \,\pm\, 0.46 }$ & $\text{--}57.4 { \scriptstyle \,\pm\, 0.76 }$ & $\text{--}6.85 { \scriptstyle \,\pm\, 0.09 }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{--}7.05 { \scriptstyle \,\pm\, 0.12 }$ & $\text{--}12.5 { \scriptstyle \,\pm\, 0.17 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.16 }$ & $\text{--}79.0 { \scriptstyle \,\pm\, 0.97 }$ & $\text{--}9.47 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $\text{--}1.21 { \scriptstyle \,\pm\, 0.02 }$ & $\text{--}3.50 { \scriptstyle \,\pm\, 0.04 }$ & $\text{--}2.68 { \scriptstyle \,\pm\, 0.05 }$ & $\text{--}2.14 { \scriptstyle \,\pm\, 0.01 }$ & $1.11 { \scriptstyle \,\pm\, 6.0\text{\textsc{e}}{\,\text{--}3} }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}14.9 { \scriptstyle \,\pm\, 0.43 }$ & $\text{--}25.0 { \scriptstyle \,\pm\, 0.54 }$ & $\text{--}26.7 { \scriptstyle \,\pm\, 0.60 }$ & $\text{--}82.9 { \scriptstyle \,\pm\, 1.04 }$ & $\text{--}10.4 { \scriptstyle \,\pm\, 0.09 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}9.62 { \scriptstyle \,\pm\, 0.17 }$ & $\text{--}15.6 { \scriptstyle \,\pm\, 0.24 }$ & $\text{--}14.0 { \scriptstyle \,\pm\, 0.26 }$ & $\text{--}89.7 { \scriptstyle \,\pm\, 1.09 }$ & $\text{--}13.1 { \scriptstyle \,\pm\, 0.06 }$ \\
\midrule\multicolumn{7}{l}{\textsc{Interpolation beyond training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}115 { \scriptstyle \,\pm\, 1.85 }$ & $\text{--}117 { \scriptstyle \,\pm\, 1.73 }$ & $\text{--}156 { \scriptstyle \,\pm\, 2.80 }$ & $\text{--}143 { \scriptstyle \,\pm\, 1.62 }$ & $\text{--}14.2 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}114 { \scriptstyle \,\pm\, 2.41 }$ & $\text{--}118 { \scriptstyle \,\pm\, 1.64 }$ & $\text{--}138 { \scriptstyle \,\pm\, 2.40 }$ & $\text{--}131 { \scriptstyle \,\pm\, 1.48 }$ & $\text{--}14.8 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}323 { \scriptstyle \,\pm\, 18.0 }$ & $\text{--}387 { \scriptstyle \,\pm\, 23.4 }$ & $\text{--}240 { \scriptstyle \,\pm\, 8.83 }$ & $\text{--}881 { \scriptstyle \,\pm\, 63.8 }$ & $\text{--}1.01\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 1.64\text{\textsc{e}}{4} }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{{NaN}} { \scriptstyle \,\pm\, \text{{NaN}} }$ & $\text{{NaN}} { \scriptstyle \,\pm\, \text{{NaN}} }$ & $\text{--}9.34\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 1.55\text{\textsc{e}}{3} }$ & $\text{--}3.71\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 313 }$ & $\text{--}7.18\text{\textsc{e}}{5} { \scriptstyle \,\pm\, 9.19\text{\textsc{e}}{5} }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}1.02\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 84.3 }$ & $\text{--}6.96\text{\textsc{e}}{5} { \scriptstyle \,\pm\, 1.03\text{\textsc{e}}{6} }$ & $\text{--}552 { \scriptstyle \,\pm\, 35.3 }$ & $\text{--}973 { \scriptstyle \,\pm\, 72.4 }$ & $\text{--}14.4 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}5.91\text{\textsc{e}}{7} { \scriptstyle \,\pm\, 3.95\text{\textsc{e}}{7} }$ & $\text{--}8.07\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 5.31\text{\textsc{e}}{4} }$ & $\text{--}2.93\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 1.08\text{\textsc{e}}{4} }$ & $\text{--}8.56\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 3.24\text{\textsc{e}}{4} }$ & $\text{--}1.12\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 6.10\text{\textsc{e}}{3} }$ \\
\midrule\multicolumn{7}{l}{\textsc{Extrapolation beyond training range}} \\[0.5em] 
ConvNP & $\gL_{\mathrm{ML}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{ML}}$ & $\text{--}120 { \scriptstyle \,\pm\, 1.87 }$ & $\text{--}119 { \scriptstyle \,\pm\, 1.73 }$ & $\text{--}138 { \scriptstyle \,\pm\, 2.36 }$ & $\text{--}131 { \scriptstyle \,\pm\, 1.43 }$ & $\text{--}14.0 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{ML}}$ & $\text{--}194 { \scriptstyle \,\pm\, 4.68 }$ & $\text{--}164 { \scriptstyle \,\pm\, 3.32 }$ & $\text{--}173 { \scriptstyle \,\pm\, 4.01 }$ & $\text{--}132 { \scriptstyle \,\pm\, 1.56 }$ & $\text{--}14.1 { \scriptstyle \,\pm\, 0.05 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{IW}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{IW}}$ & $\text{--}567 { \scriptstyle \,\pm\, 6.18 }$ & $\text{--}691 { \scriptstyle \,\pm\, 8.56 }$ & $\text{--}567 { \scriptstyle \,\pm\, 7.17 }$ & $\text{--}1.48\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 36.4 }$ & $\text{--}540 { \scriptstyle \,\pm\, 5.93 }$ \\
NP & $\gL_{\mathrm{IW}}$ & $\text{--}2.19\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 51.9 }$ & $\text{--}704 { \scriptstyle \,\pm\, 11.4 }$ & $\text{--}4.00\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 113 }$ & $\text{--}3.64\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 105 }$ & $\text{--}54.8 { \scriptstyle \,\pm\, 0.46 }$ \\[.5em]
ConvNP & $\gL_{\mathrm{NP}}$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ & $0.00 { \scriptstyle \,\pm\, 0.00 }$ \\
ANP & $\gL_{\mathrm{NP}}$ & $\text{--}2.52\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 60.7 }$ & $\text{--}8.59\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 256 }$ & $\text{--}1.43\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 42.2 }$ & $\text{--}1.11\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 36.3 }$ & $\text{--}14.1 { \scriptstyle \,\pm\, 0.05 }$ \\
NP & $\gL_{\mathrm{NP}}$ & $\text{--}6.75\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 266 }$ & $\text{--}1.93\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 702 }$ & $\text{--}1.12\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 41.4 }$ & $\text{--}1.04\text{\textsc{e}}{4} { \scriptstyle \,\pm\, 440 }$ & $\text{--}1.58\text{\textsc{e}}{3} { \scriptstyle \,\pm\, 30.9 }$ \\
\bottomrule

\end{tabular}
\end{center}
\end{table}


==> tables/bakeoff_main_text.tex <==
\begin{table}[t]
\footnotesize
\caption{Log-likelihood of ConvNP and ANP trained with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$ on 1D regression tasks.}
\label{table:1d_bakeoff_main_text}
\begin{center}
\begin{tabular}{@{}l@{\hspace{4pt}}
                c@{\hspace{4pt}}
                c@{\hspace{6pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{}}

\toprule 
 & & &
 \multicolumn{3}{c}{\textsc{within training range}} & 
 \multicolumn{3}{c}{\textsc{beyond training range}}\\
 \midrule
 & \textsc{train} & \textsc{eval} &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  & 
 \multicolumn{1}{c}{Weakly Per.}         & 
 \multicolumn{1}{c}{Sawtooth}            &
 \multicolumn{1}{c}{Mat\'ern-$\frac52$}  &
 \multicolumn{1}{c}{Weakly Per.}         &
 \multicolumn{1}{c}{Sawtooth}\\
 \midrule
 %
 ConvNP & $\gL_{\mathrm{ML}}$ & ML & 
 $\textbf{\text{--}0.80} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$ &         %   Matern Interpolation
 $\textbf{\text{--}1.08} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Interpolation 
 $\textbf{1.22} { \scriptstyle \,\pm\, 0.01 }$                                               &         %   Sawtooth Interpolation 
 $\textbf{\text{--}0.80} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$ &         %   Matern Extrapolation
 $\textbf{\text{--}1.08} { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &         %   Weakly Per. Extrapolation 
 $\textbf{1.23} { \scriptstyle \,\pm\, 0.01 }$ \\                    %   Sawtooth Extrapolation 
 %
 ANP & $\gL_{\mathrm{ML}}$ & ML & 
 $\text{--}0.90 { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Interpolation
 $\text{--}1.20 { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $\text{--}0.03 { \scriptstyle \,\pm\, 3\text{\textsc{e}}{\,\text{--}3} }$ &        %   Sawtooth Interpolation
 $\text{--}1.30 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Extrapolation
 $\text{--}1.34 { \scriptstyle \,\pm\, 5\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Extrapolation
 $\text{--}0.20 { \scriptstyle \,\pm\, 2\text{\textsc{e}}{\,\text{--}3} }$ \\ %   Sawtooth Extrapolation
 %
 \midrule
 %
 ConvNP & $\gL_{\mathrm{NP}}$ & IW &
 $\textbf{\text{--}0.89} { \scriptstyle \,\pm\, 0.01 }$          &     %   Matern Interpolation
 $\textbf{\text{--}1.11} { \scriptstyle \,\pm\, 0.01 }$ &     %   Weakly Per.
 $\textbf{1.53} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$          &     %   Sawtooth Interpolation
 $\textbf{\text{--}0.89} { \scriptstyle \,\pm\, 0.03 }$          &     %   Matern Extrapolation
 $\textbf{\text{--}1.10} { \scriptstyle \,\pm\, 0.01 }$ &     %   Weakly Per. Extrapolation
 $\textbf{1.52} { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 ANP & $\gL_{\mathrm{NP}}$ & IW &
 $\text{--}0.95 { \scriptstyle \,\pm\, 8\text{\textsc{e}}{\,\text{--}3} }$ &        %   Matern Interpolation
 $\text{--}1.18 { \scriptstyle \,\pm\, 6\text{\textsc{e}}{\,\text{--}3} }$ &        %   Weakly Per. Interpolation
 $\text{--}0.02 { \scriptstyle \,\pm\, 4\text{\textsc{e}}{\,\text{--}3} }$ &        %   Sawtooth Interpolation
 $\text{--}4.09 { \scriptstyle \,\pm\, 0.18 }$                             &        %   Matern Extrapolation
 $\text{--}1.60 { \scriptstyle \,\pm\, 0.02 }$                             &        %   Weakly Per. Extrapolation
 $\text{--}0.19 { \scriptstyle \,\pm\, 2\text{\textsc{e}}{\,\text{--}3} }$ \\       %   Sawtooth Extrapolation
 %
 \midrule
 %
  ConvCNP & & &
 $\text{--}{0.88} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Interpolation
 $\text{--}{1.18} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$                                    &         %   Weakly Per. Interpolation 
 $1.15 { \scriptstyle \,\pm\, 0.05 }$                                               &         %   Sawtooth Interpolation 
 $\text{--}{0.88} { \scriptstyle \,\pm\, 0.01 }$                                    &         %   Matern Extrapolation
 $\text{--}{1.18} { \scriptstyle \,\pm\, 7\text{\textsc{e}}{\,\text{--}3} }$                                    &         %   Weakly Per. Extrapolation 
 $1.14 { \scriptstyle \,\pm\, 0.04 }$ \\                    %   Sawtooth Extrapolation 
 %
 \bottomrule

\end{tabular}
\end{center}
\end{table}


==> tables/environmental_metrics.tex <==
\begin{table}[htb] 
\vspace*{-0.5em}
\caption{Average joint predictive log-likelihood (LL) and RMSE on ERA5Land. }
\label{table:era5_loglik_rmse}
\begin{center}
\begin{tabular}{
    l@{\hspace{4pt}}
    l@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}
    r@{\hspace{4pt}}c}
\toprule 
 & &
 \multicolumn{1}{r}{Central (train)} & 
 \multicolumn{1}{r}{West (test)} & 
 \multicolumn{1}{r}{East (test)} & 
 \multicolumn{1}{r}{South (test)}\\
 %
 \midrule 
 %
 LL &  ConvNP  & 
 $\textbf{6.16} { \scriptstyle \,\pm\, 0.098 }$ & 
 $\textbf{5.87} { \scriptstyle \,\pm\, 0.104 }$ & 
 $\textbf{6.78} { \scriptstyle \,\pm\, 0.106 }$ & 
 $\textbf{8.51} { \scriptstyle \,\pm\, 0.169 }$ \\
 %
 & GP & 
 $4.95 { \scriptstyle \,\pm\, 0.072 }$ & 
 $4.89 { \scriptstyle \,\pm\, 0.087 }$ & 
 $5.31 { \scriptstyle \,\pm\, 0.100 }$ & 
 $6.23 { \scriptstyle \,\pm\, 0.109 }$ \\[.5em]
 %
 RMSE & ConvNP & 
 $\textbf{2.13}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.34\text{\textsc{e}}{-4} }$ &
 $\textbf{2.62}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 3.55\text{\textsc{e}}{-4} }$ & 
 $\textbf{1.18}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.32\text{\textsc{e}}{-4} }$ & 
 $6.79\text{\textsc{e}}{-4} { \scriptstyle \,\pm\, 8.14\text{\textsc{e}}{-5} }$ \\
 %
  & GP & 
 $2.50\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.59\text{\textsc{e}}{-4} }$ & 
 $\textbf{2.21}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 1.34\text{\textsc{e}}{-4} }$ & 
 $\textbf{1.13}\text{\textsc{e}}{-3} { \scriptstyle \,\pm\, 4.60\text{\textsc{e}}{-5} }$ &
 $\textbf{4.10}\text{\textsc{e}}{-4} { \scriptstyle \,\pm\, 3.49\text{\textsc{e}}{-5} }$ \\
 \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/image_main_text_squeeze_hetero.tex <==
\begin{table}[t]
\footnotesize
\caption{Test log-likelihood lower bounds for image completion (5 runs).}
\label{table:images_main_text}
\vspace*{-2pt}
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{} & 
\multicolumn{2}{c}{MNIST}                 & 
\multicolumn{2}{c}{CelebA32}              & 
\multicolumn{2}{c}{SVHN}                  & 
\multicolumn{2}{c}{ZSMM}                  \\ 
%
& 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ &  $\gL_{\mathrm{NP}}$ & 
$\gL_{\mathrm{ML}}$ & $\gL_{\mathrm{NP}}$ \\ 
%
\midrule
%
ConvNP    &  
$1.28 { \scriptstyle \,\pm\, 0.00 }$  &   % MNIST ML
$1.16 { \scriptstyle \,\pm\, 0.16 }$           &   % MNIST NP                 
$\textbf{6.92} { \scriptstyle \,\pm\, 0.10 }$  &   % CELEBA ML              
$-0.27 { \scriptstyle \,\pm\, 0.00 }$           &   % CELEBA NP
$\textbf{9.89} { \scriptstyle \,\pm\, 0.09}$   &   % SVHN ML                   
$0.17 { \scriptstyle \,\pm\, 0.00 }$           &   % SVHN NP                   
$\textbf{3.75} { \scriptstyle \,\pm\, 0.01 }$  &   % ZSMM ML
$0.13  { \scriptstyle \,\pm\, 0.00}$           \\  % ZSMM NP
%
ANP   &
$1.26 { \scriptstyle \,\pm\, 0.00 }$           &  % MNIST ML
$\textbf{1.29} { \scriptstyle \,\pm\, 0.00 }$           &  % MNIST NP           
$5.98 { \scriptstyle \,\pm\, 0.08 }$           &  % CELEBA ML         
$6.04 { \scriptstyle \,\pm\, 0.10 }$           &  % CELEBA NP         
$9.18 { \scriptstyle \,\pm\, 0.08 }$           &  % SVHN ML         
$8.91 { \scriptstyle \,\pm\, 0.06 }$           &  % SVHN NP         
$-2.03 { \scriptstyle \,\pm\, 0.08 }$           &  % ZSMM ML         
$-2.13 { \scriptstyle \,\pm\, 0.27 }$           \\ % ZSMM NP
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\vspace*{-1.0em}
\end{table}

% NOTE : here all the models are heteroskedastic

==> tables/images_main_text.tex <==
\begin{table}[htb]
\begin{center}
\caption{Per-pixel test log-likelihood of ConvNP and ANP trained with $\gL_{\mathrm{ML}}$ and $\gL_{\mathrm{NP}}$ (5 runs).}
\label{table:images_main_text}
\begin{tabular}{l@{\hspace{4pt}}
                l@{\hspace{6pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{4pt}}
                r@{\hspace{0pt}}}

\toprule 
 & & 
 \multicolumn{1}{c}{MNIST} & 
 \multicolumn{1}{c}{CelebA32}         & 
 \multicolumn{1}{c}{SVHN}           &
 \multicolumn{1}{c}{ZSMM}           \\
 \midrule
 %
 ConvNP & $\gL_{\mathrm{ML}}$ & 
 $\textbf{2.03} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   MNIST
 $\textbf{4.11} { \scriptstyle \,\pm\, 0.01 }$ &                                     %   CELEBA
 $\textbf{8.35} { \scriptstyle \,\pm\, 0.05}$ &         %   SVHN
 $\textbf{1.39} { \scriptstyle \,\pm\, 0.03 }$ \\[.2em]                                    %   ZSMM
 %
 ConvNP & $\gL_{\mathrm{NP}}$ &
 $1.02 { \scriptstyle \,\pm\, 0.00 }$ &     %   MNIST
 $2.13 { \scriptstyle \,\pm\, 0.12  }$ &     %   CELEBA
 $4.71 { \scriptstyle \,\pm\, 0.02 }$          &     %   SVHN
 $0.04  { \scriptstyle \,\pm\, 0.00}$ \\[.2em]      %   ZSMM
 %
 ANP & $\gL_{\mathrm{ML}}$ & 
 $1.82 { \scriptstyle \,\pm\, 0.01 }$ &                                    %   MNIST
 $3.72 { \scriptstyle \,\pm\, 0.02 }$ &                                             %   CELEBA
 $7.71 { \scriptstyle \,\pm\, 0.03 }$          &        %   SVHN
 $0.42 { \scriptstyle \,\pm\, 0.03 }$  \\[.2em]        %   ZSMM 
 %
 ANP & $\gL_{\mathrm{NP}}$ &
 $1.05 { \scriptstyle \,\pm\, 0.07 }$ &                                    %   MNIST
 $3.57 { \scriptstyle \,\pm\, 0.02 }$ &        %   CELEBA
 $7.62 { \scriptstyle \,\pm\,  0.05}$          &        %   SVHN
 $0.24 { \scriptstyle \,\pm\, 0.04 }$ \\         %   ZSMM
 \bottomrule

\end{tabular}
\end{center}
\end{table}

